Spectroscopy of $NbSe_2$ using Energy-Tunable Defect-Embedded Quantum Dots

Quantum dots have sharply defined energy levels, which can be used for high resolution energy spectroscopy when integrated in tunneling circuitry. Here we report dot-assisted spectroscopy measurements of the superconductor $NbSe_2$, using a van der Waals device consisting of a vertical stack of $graphene-MoS_2-NbSe_2$. The $MoS_2$ tunnel barriers host naturally occurring defects which function as quantum dots, allowing transport via resonant tunneling. The dot energies are tuned by an electric field exerted by a back-gate, which penetrates the graphene source electrode. Scanning the dot potential across the superconductor Fermi energy, we reproduce the $NbSe_2$ density of states which exhibits a well-resolved two-gap spectrum. Surprisingly, we find that the dot-assisted current is dominated by the lower energy feature of the two $NbSe_2$ gaps, possibly due to a selection rule which favors coupling between the dots and the orbitals which exhibit this gap.

==> References.tex <==
\providecommand{\latin}[1]{#1}
\makeatletter
\providecommand{\doi}
  {\begingroup\let\do\@makeother\dospecials
  \catcode`\{=1 \catcode`\}=2 \doi@aux}
\providecommand{\doi@aux}[1]{\endgroup\texttt{#1}}
\makeatother
\providecommand*\mcitethebibliography{\thebibliography}
\csname @ifundefined\endcsname{endmcitethebibliography}
  {\let\endmcitethebibliography\endthebibliography}{}
\begin{mcitethebibliography}{40}
\providecommand*\natexlab[1]{#1}
\providecommand*\mciteSetBstSublistMode[1]{}
\providecommand*\mciteSetBstMaxWidthForm[2]{}
\providecommand*\mciteBstWouldAddEndPuncttrue
  {\def\EndOfBibitem{\unskip.}}
\providecommand*\mciteBstWouldAddEndPunctfalse
  {\let\EndOfBibitem\relax}
\providecommand*\mciteSetBstMidEndSepPunct[3]{}
\providecommand*\mciteSetBstSublistLabelBeginEnd[3]{}
\providecommand*\EndOfBibitem{}
\mciteSetBstSublistMode{f}
\mciteSetBstMaxWidthForm{subitem}{(\alph{mcitesubitemcount})}
\mciteSetBstSublistLabelBeginEnd
  {\mcitemaxwidthsubitemform\space}
  {\relax}
  {\relax}

\bibitem[Giaever(1960)]{Giaever1960}
Giaever,~I. {Energy gap in superconductors measured by electron tunneling}.
  \emph{Phys. Rev. Lett.} \textbf{1960}, \emph{5}, 147--148\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[Dvir \latin{et~al.}(2018)Dvir, Massee, Attias, Khodas, Aprili, Quay,
  and Steinberg]{Dvir2018}
Dvir,~T.; Massee,~F.; Attias,~L.; Khodas,~M.; Aprili,~M.; Quay,~C.~H.;
  Steinberg,~H. {Spectroscopy of bulk and few-layer superconducting $NbSe_2$
  with van der Waals tunnel junctions}. \emph{Nat. Commun.} \textbf{2018},
  \emph{9}, 598\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[Dvir \latin{et~al.}(2018)Dvir, Aprili, Quay, and Steinberg]{Dvir2018a}
Dvir,~T.; Aprili,~M.; Quay,~C.~H.; Steinberg,~H. {Tunneling into the Vortex
  State of $NbSe_2$ with van der Waals Junctions}. \emph{Nano Lett.}
  \textbf{2018}, \emph{18}, 7845--7850\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[Zalic \latin{et~al.}(2019)Zalic, Simon, Remennik, Vakahi, Gu, and
  Steinberg]{Zalic2019}
Zalic,~A.; Simon,~S.; Remennik,~S.; Vakahi,~A.; Gu,~G.~D.; Steinberg,~H.
  {$FeTe_{0.55}Se_{0.45}$ van der Waals tunneling devices}. \emph{Phys. Rev. B}
  \textbf{2019}, \emph{100}, 064517\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[Britnell \latin{et~al.}(2012)Britnell, Gorbachev, Jalil, Belle,
  Schedin, Katsnelson, Eaves, Morozov, Mayorov, Peres, {Castro Neto}, Leist,
  Geim, Ponomarenko, and Novoselov]{Britnell2012}
Britnell,~L.; Gorbachev,~R.~V.; Jalil,~R.; Belle,~B.~D.; Schedin,~F.;
  Katsnelson,~M.~I.; Eaves,~L.; Morozov,~S.~V.; Mayorov,~A.~S.; Peres,~N.~M.;
  {Castro Neto},~A.~H.; Leist,~J.; Geim,~A.~K.; Ponomarenko,~L.~A.;
  Novoselov,~K.~S. {Electron tunneling through ultrathin boron nitride
  crystalline barriers}. \emph{Nano Lett.} \textbf{2012}, \emph{12},
  1707--1710\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[Greibe \latin{et~al.}(2011)Greibe, Stenberg, Wilson, Bauch, Shumeiko,
  and Delsing]{Greibe2011}
Greibe,~T.; Stenberg,~M.~P.; Wilson,~C.~M.; Bauch,~T.; Shumeiko,~V.~S.;
  Delsing,~P. {Are "pinholes" the cause of excess current in superconducting
  tunnel junctions? A study of Andreev current in highly resistive junctions}.
  \emph{Phys. Rev. Lett.} \textbf{2011}, \emph{106}, 097001\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[Island \latin{et~al.}(2016)Island, Steele, {Van Der Zant}, and
  Castellanos-Gomez]{Island2016}
Island,~J.~O.; Steele,~G.~A.; {Van Der Zant},~H.~S.; Castellanos-Gomez,~A.
  {Thickness dependent interlayer transport in vertical $MoS_2$ Josephson
  junctions}. \emph{2D Mater.} \textbf{2016}, \emph{3}, 031002\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[Chakraborty \latin{et~al.}(2015)Chakraborty, Kinnischtzke, Goodfellow,
  Beams, and Vamivakas]{Chakraborty2015}
Chakraborty,~C.; Kinnischtzke,~L.; Goodfellow,~K.~M.; Beams,~R.;
  Vamivakas,~A.~N. {Voltage-controlled quantum light from an atomically thin
  semiconductor}. \emph{Nat. Nanotechnol.} \textbf{2015}, \emph{10},
  507--511\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[He \latin{et~al.}(2015)He, Clark, Schaibley, He, Chen, Wei, Ding,
  Zhang, Yao, Xu, Lu, and Pan]{He2015}
He,~Y.~M.; Clark,~G.; Schaibley,~J.~R.; He,~Y.; Chen,~M.~C.; Wei,~Y.~J.;
  Ding,~X.; Zhang,~Q.; Yao,~W.; Xu,~X.; Lu,~C.~Y.; Pan,~J.~W. {Single quantum
  emitters in monolayer semiconductors}. \emph{Nat. Nanotechnol.}
  \textbf{2015}, \emph{10}, 497--502\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[Tran \latin{et~al.}(2016)Tran, Elbadawi, Totonjian, Lobo, Grosso,
  Moon, Englund, Ford, Aharonovich, and Toth]{Tran2017}
Tran,~T.~T.; Elbadawi,~C.; Totonjian,~D.; Lobo,~C.~J.; Grosso,~G.; Moon,~H.;
  Englund,~D.~R.; Ford,~M.~J.; Aharonovich,~I.; Toth,~M. {Robust multicolor
  single photon emission from point defects in hexagonal boron nitride}.
  \emph{ACS Nano} \textbf{2016}, \emph{10}, 7331--7338\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[Hong \latin{et~al.}(2015)Hong, Hu, Probert, Li, Lv, Yang, Gu, Mao,
  Feng, Xie, Zhang, Wu, Zhang, Jin, Ji, Zhang, Yuan, and Zhang]{Hong2015}
Hong,~J. \latin{et~al.}  {Exploring atomic defects in molybdenum disulphide
  monolayers}. \emph{Nat. Commun.} \textbf{2015}, \emph{6}, 6293\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[Vancs{\'{o}} \latin{et~al.}(2016)Vancs{\'{o}}, Magda, Peto, Noh, Kim,
  Hwang, Bir{\'{o}}, and Tapaszt{\'{o}}]{Vancso2016}
Vancs{\'{o}},~P.; Magda,~G.~Z.; Peto,~J.; Noh,~J.~Y.; Kim,~Y.~S.; Hwang,~C.;
  Bir{\'{o}},~L.~P.; Tapaszt{\'{o}},~L. {The intrinsic defect structure of
  exfoliated $MoS_2$ single layers revealed by Scanning Tunneling Microscopy}.
  \emph{Sci. Rep.} \textbf{2016}, \emph{6}, 29726\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[Chandni \latin{et~al.}(2015)Chandni, Watanabe, Taniguchi, and
  Eisenstein]{Chandni2015}
Chandni,~U.; Watanabe,~K.; Taniguchi,~T.; Eisenstein,~J.~P. {Evidence for
  Defect-Mediated Tunneling in Hexagonal Boron Nitride-Based Junctions}.
  \emph{Nano Lett.} \textbf{2015}, \emph{15}, 7329--7333\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[Greenaway \latin{et~al.}(2018)Greenaway, Vdovin, Ghazaryan, Misra,
  Mishchenko, Cao, Wang, Wallbank, Holwill, Khanin, Morozov, Watanabe,
  Taniguchi, Makarovsky, Fromhold, Patan{\`{e}}, Geim, Fal'ko, Novoselov, and
  Eaves]{Greenaway2018}
Greenaway,~M.~T. \latin{et~al.}  {Tunnel spectroscopy of localised electronic
  states in hexagonal boron nitride}. \emph{Commun. Phys.} \textbf{2018},
  \emph{1}, 94\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[Papadopoulos \latin{et~al.}(2020)Papadopoulos, Gehring, Watanabe,
  Taniguchi, {Van Der Zant}, and Steele]{Papadopoulos2020}
Papadopoulos,~N.; Gehring,~P.; Watanabe,~K.; Taniguchi,~T.; {Van Der
  Zant},~H.~S.; Steele,~G.~A. {Tunneling spectroscopy of localized states of
  $WS_2$ barriers in vertical van der Waals heterostructures}. \emph{Phys. Rev.
  B} \textbf{2020}, \emph{101}, 165303\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[Keren \latin{et~al.}(2020)Keren, Dvir, Zalic, Iluz, LeBoeuf, Watanabe,
  Taniguchi, and Steinberg]{Keren2020}
Keren,~I.; Dvir,~T.; Zalic,~A.; Iluz,~A.; LeBoeuf,~D.; Watanabe,~K.;
  Taniguchi,~T.; Steinberg,~H. {Quantum-dot assisted spectroscopy of
  degeneracy-lifted Landau levels in graphene}. \emph{Nat. Commun.}
  \textbf{2020}, \emph{11}, 3408\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[Dvir \latin{et~al.}(2019)Dvir, Aprili, Quay, and Steinberg]{Dvir2019}
Dvir,~T.; Aprili,~M.; Quay,~C.~H.; Steinberg,~H. {Zeeman Tunability of Andreev
  Bound States in van der Waals Tunnel Barriers}. \emph{Phys. Rev. Lett.}
  \textbf{2019}, \emph{123}, 217003\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[{De Franceschi} \latin{et~al.}(2010){De Franceschi}, Kouwenhoven,
  Sch{\"{o}}nenberger, and Wernsdorfer]{DeFranceschi2010}
{De Franceschi},~S.; Kouwenhoven,~L.; Sch{\"{o}}nenberger,~C.; Wernsdorfer,~W.
  {Hybrid superconductor-quantum dot devices}. \emph{Nat. Nanotechnol.}
  \textbf{2010}, \emph{5}, 703--711\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[Deacon \latin{et~al.}(2010)Deacon, Tanaka, Oiwa, Sakano, Yoshida,
  Shibata, Hirakawa, and Tarucha]{Deacon2010}
Deacon,~R.~S.; Tanaka,~Y.; Oiwa,~A.; Sakano,~R.; Yoshida,~K.; Shibata,~K.;
  Hirakawa,~K.; Tarucha,~S. {Kondo-enhanced Andreev transport in single
  self-assembled InAs quantum dots contacted with normal and superconducting
  leads}. \emph{Phys. Rev. B} \textbf{2010}, \emph{81}, 121308\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[Lee \latin{et~al.}(2014)Lee, Jiang, Houzet, Aguado, Lieber, and {De
  Franceschi}]{Lee2014}
Lee,~E.~J.; Jiang,~X.; Houzet,~M.; Aguado,~R.; Lieber,~C.~M.; {De
  Franceschi},~S. {Spin-resolved Andreev levels and parity crossings in hybrid
  superconductor-semiconductor nanostructures}. \emph{Nat. Nanotechnol.}
  \textbf{2014}, \emph{9}, 79--84\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[Scher{\"{u}}bl \latin{et~al.}(2020)Scher{\"{u}}bl, F{\"{u}}l{\"{o}}p,
  Moca, Gramich, Baumgartner, Makk, Elalaily, Sch{\"{o}}nenberger, Nyg{\aa}rd,
  Zar{\'{a}}nd, and Csonka]{Scherubl2020}
Scher{\"{u}}bl,~Z.; F{\"{u}}l{\"{o}}p,~G.; Moca,~C.~P.; Gramich,~J.;
  Baumgartner,~A.; Makk,~P.; Elalaily,~T.; Sch{\"{o}}nenberger,~C.;
  Nyg{\aa}rd,~J.; Zar{\'{a}}nd,~G.; Csonka,~S. {Large spatial extension of the
  zero-energy Yu–Shiba–Rusinov state in a magnetic field}. \emph{Nat.
  Commun.} \textbf{2020}, \emph{11}, 1834\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[Deng \latin{et~al.}(2016)Deng, Vaitiekenas, Hansen, Danon, Leijnse,
  Flensberg, Nyg{\aa}rd, Krogstrup, and Marcus]{Deng2016}
Deng,~M.~T.; Vaitiekenas,~S.; Hansen,~E.~B.; Danon,~J.; Leijnse,~M.;
  Flensberg,~K.; Nyg{\aa}rd,~J.; Krogstrup,~P.; Marcus,~C.~M. {Majorana bound
  state in a coupled quantum-dot hybrid-nanowire system}. \emph{Science}
  \textbf{2016}, \emph{354}, 1557--1562\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[J{\"{u}}nger \latin{et~al.}(2019)J{\"{u}}nger, Baumgartner,
  Delagrange, Chevallier, Lehmann, Nilsson, Dick, Thelander, and
  Sch{\"{o}}nenberger]{Junger2019}
J{\"{u}}nger,~C.; Baumgartner,~A.; Delagrange,~R.; Chevallier,~D.; Lehmann,~S.;
  Nilsson,~M.; Dick,~K.~A.; Thelander,~C.; Sch{\"{o}}nenberger,~C.
  {Spectroscopy of the superconducting proximity effect in nanowires using
  integrated quantum dots}. \emph{Commun. Phys.} \textbf{2019}, \emph{2},
  76\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[Wang \latin{et~al.}(2018)Wang, Bretheau, Rodan-Legrain, Pisoni,
  Watanabe, Taniguchi, and Jarillo-Herrero]{Wang2018}
Wang,~J.~I.; Bretheau,~L.; Rodan-Legrain,~D.; Pisoni,~R.; Watanabe,~K.;
  Taniguchi,~T.; Jarillo-Herrero,~P. {Tunneling spectroscopy of graphene
  nanodevices coupled to large-gap superconductors}. \emph{Phys. Rev. B}
  \textbf{2018}, \emph{98}, 121411\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[Boaknin \latin{et~al.}(2004)Boaknin, Tanatar, Paglione, Hawthorn,
  Hill, Ronning, Sutherland, Taillefer, Sonier, Hayden, and Brill]{Boaknin2004}
Boaknin,~E.; Tanatar,~M.~A.; Paglione,~J.; Hawthorn,~D.~G.; Hill,~R.~W.;
  Ronning,~F.; Sutherland,~M.; Taillefer,~L.; Sonier,~J.; Hayden,~S.~M.;
  Brill,~J.~W. {Multi-band superconductivity in $NbSe_2$ from heat transport}.
  \emph{Phys. C: Superconductivity} \textbf{2004}, \emph{408-410},
  727--728\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[Zehetmayer and Weber(2010)Zehetmayer, and Weber]{Zehetmayer2010}
Zehetmayer,~M.; Weber,~H.~W. {Experimental evidence for a two-band
  superconducting state of $NbSe_2$ single crystals}. \emph{Phys. Rev. B}
  \textbf{2010}, \emph{82}, 014524\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[Noat \latin{et~al.}(2015)Noat, Silva-Guill{\'{e}}n, Cren, Cherkez,
  Brun, Pons, Debontridder, Roditchev, Sacks, Cario, Ordej{\'{o}}n,
  Garc{\'{i}}a, and Canadell]{Noat2015}
Noat,~Y.; Silva-Guill{\'{e}}n,~J.~A.; Cren,~T.; Cherkez,~V.; Brun,~C.;
  Pons,~S.; Debontridder,~F.; Roditchev,~D.; Sacks,~W.; Cario,~L.;
  Ordej{\'{o}}n,~P.; Garc{\'{i}}a,~A.; Canadell,~E. {Quasiparticle spectra of
  $2H-NbSe_2$: Two-band superconductivity and the role of tunneling
  selectivity}. \emph{Phys. Rev. B} \textbf{2015}, \emph{92}, 134510\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[Momma and Izumi(2011)Momma, and Izumi]{Momma2011}
Momma,~K.; Izumi,~F. {VESTA 3 for three-dimensional visualization of crystal,
  volumetric and morphology data}. \emph{J. Appl. Cryst.} \textbf{2011},
  \emph{44}, 1272--1276\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[Castellanos-Gomez \latin{et~al.}(2014)Castellanos-Gomez, Buscema,
  Molenaar, Singh, Janssen, {Van Der Zant}, and Steele]{Castellanos-Gomez2014}
Castellanos-Gomez,~A.; Buscema,~M.; Molenaar,~R.; Singh,~V.; Janssen,~L.; {Van
  Der Zant},~H.~S.; Steele,~G.~A. {Deterministic transfer of two-dimensional
  materials by all-dry viscoelastic stamping}. \emph{2D Mater.} \textbf{2014},
  \emph{1}, 011002\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[Tinkham(2004)]{Tinkham2004}
Tinkham,~M. \emph{Introduction To Superconductivity}; Dover Publications, Inc.:
  New York, 2004\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[Bardeen(1961)]{Bardeen1961}
Bardeen,~J. {Tunneling from a many-particle point of view}. \emph{Phys. Rev.
  Lett.} \textbf{1961}, \emph{6}, 57--59\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[McMillan(1968)]{McMillan1968}
McMillan,~W.~L. {Tunneling Model of the Superconducting Proximity Effect}.
  \emph{Phys. Rev} \textbf{1968}, \emph{175}, 537--542\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[Kiss \latin{et~al.}(2007)Kiss, Yokoya, Chainani, Shin, Hanaguri,
  Nohara, and Takagi]{Kiss2007}
Kiss,~T.; Yokoya,~T.; Chainani,~A.; Shin,~S.; Hanaguri,~T.; Nohara,~M.;
  Takagi,~H. {Charge-order-maximized momentum-dependent superconductivity}.
  \emph{Nat. Phys.} \textbf{2007}, \emph{3}, 720--725\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[Suhl \latin{et~al.}(1959)Suhl, Matthias, and Walker]{Suhl1959}
Suhl,~H.; Matthias,~B.~T.; Walker,~L.~R. {Bardeen-Cooper-Schrieffer theory in
  the case of overlapping bands}. \emph{Phys. Rev. Lett.} \textbf{1959},
  \emph{3}, 552--554\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[Schopohl and Scharnberg(1977)Schopohl, and Scharnberg]{Schopohl1977}
Schopohl,~N.; Scharnberg,~K. {Tunneling density of states for the two-band
  model of superconductivity}. \emph{Solid State Commun.} \textbf{1977},
  \emph{22}, 371--374\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[Guillamon \latin{et~al.}(2008)Guillamon, Suderow, Guinea, and
  Vieira]{Guillamon2008}
Guillamon,~I.; Suderow,~H.; Guinea,~F.; Vieira,~S. {Intrinsic atomic-scale
  modulations of the superconducting gap of $2H-NbSe_2$}. \emph{Phys. Rev. B}
  \textbf{2008}, \emph{77}, 134505\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[Noat \latin{et~al.}(2010)Noat, Cren, Debontridder, Roditchev, Sacks,
  Toulemonde, and {San Miguel}]{Noat2010}
Noat,~Y.; Cren,~T.; Debontridder,~F.; Roditchev,~D.; Sacks,~W.; Toulemonde,~P.;
  {San Miguel},~A. {Signatures of multigap superconductivity in tunneling
  spectroscopy}. \emph{Phys. Rev. B} \textbf{2010}, \emph{82}, 014531\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[Rahn \latin{et~al.}(2012)Rahn, Hellmann, Kall{\"{a}}ne, Sohrt, Kim,
  Kipp, and Rossnagel]{Rahn2012}
Rahn,~D.~J.; Hellmann,~S.; Kall{\"{a}}ne,~M.; Sohrt,~C.; Kim,~T.~K.; Kipp,~L.;
  Rossnagel,~K. {Gaps and kinks in the electronic structure of the
  superconductor $2H-NbSe_2$ from angle-resolved photoemission at 1 K}.
  \emph{Phys. Rev. B} \textbf{2012}, \emph{85}, 224532\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem[Qiu \latin{et~al.}(2013)Qiu, Xu, Wang, Ren, Nan, Ni, Chen, Yuan, Miao,
  Song, Long, Shi, Sun, Wang, and Wang]{Qiu2013}
Qiu,~H.; Xu,~T.; Wang,~Z.; Ren,~W.; Nan,~H.; Ni,~Z.; Chen,~Q.; Yuan,~S.;
  Miao,~F.; Song,~F.; Long,~G.; Shi,~Y.; Sun,~L.; Wang,~J.; Wang,~X. {Hopping
  transport through defect-induced localized states in molybdenum disulphide}.
  \emph{Nat. Commun.} \textbf{2013}, \emph{4}, 2642\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\end{mcitethebibliography}

